Local Nash Equilibria are Isolated, Strict Local Nash Equilibria in `Almost All' Zero-Sum Continuous Games

We prove that differential Nash equilibria are generic amongst local Nash equilibria in continuous zero-sum games. That is, there exists an open-dense subset of zero-sum games for which local Nash equilibria are non-degenerate differential Nash equilibria. The result extends previous results to the zero-sum setting, where we obtain even stronger results; in particular, we show that local Nash equilibria are generically hyperbolic critical points. We further show that differential Nash equilibria of zero-sum games are structurally stable. The purpose for presenting these extensions is the recent renewed interest in zero-sum games within machine learning and optimization. Adversarial learning and generative adversarial network approaches are touted to be more robust than the alternative. Zero-sum games are at the heart of such approaches. Many works proceed under the assumption of hyperbolicity of critical points. Our results justify this assumption by showing `almost all' zero-sum games admit local Nash equilibria that are hyperbolic.

==> [2019 CDC] Zero Sum Genericity (1)/conclusion.tex <==
\section{Discussion and Concluding Remarks}
\label{sec:conclusion}
The focus of this paper is on the genericity and structural stability of a particular refinement of the local Nash equilibrium concept---namely, differential Nash equilibria---within the class of two-player, zero-sum continuous games. 
The renewed interest in zero-sum games on continuous action spaces is primarily due to the widespread adoption of game theoretic tools in areas such as robust reinforcement learning and adversarial learning including generative adversarial networks. 
For instance, zero-sum continuous game abstractions have shown to be particularly adept at learning robust policies for a wide-variety of tasks from classification to prediction to control.

Most learning approaches are based on local information such as gradient updates, and as such, representations of Nash equilibria that are amenable to computation such as the differential Nash concept are extremely relevant. Much of the existing convergence analysis for machine learning algorithms based on game-theoretic concepts proceeds under the structural assumptions implicit in the definition of the differential Nash equilibrium concept. In this paper, we show that characterizations such as these are generic and structurally stable; hence, the aforementioned structural assumptions only rule out a measure zero set of games, and the desired properties are robust to smooth perturbations in player costs.
%These results help to justify assumpti
%In this paper, we focus on showing that a refinement---i.e., differential Nash---of the local Nash equilibrium concept with a structure that is particularly amenable to computation since it is characterized in terms of local information is generic. That is, local Nash equilibria are generically differential Nash equilibria and hence, the structure of differential Nash equilibria can be taken advantage of in both computation and learning regimes.


==> [2019 CDC] Zero Sum Genericity (1)/game_prelims.tex <==
\subsection{Preliminary Definitions}
\label{sec:setup}

In this paper, we consider full information continuous, two-player zero-sum games.
We use the term `player' and `agent' interchangeably. 
Each player $i\in \mc{I}=\{1,2\}$ selects an action $x_i$ from a
\emph{topological space} $X_i$ in order to minimize its cost $f_i:X\rar \mb{R}$
where $X=X_1\times X_2$ is the \emph{joint strategy space} of all the
agents. Note that $f_i$ depends on $x_{-i}$
%\[x_{-i}=(x_1, \ldots,
%x_{i-1}, x_{i+1}, \ldots, x_n)=(x_j)_{j\in \mc{I}/\{i\}}\]
which is the collection of actions of all other agents excluding agent
$i$---that is, $f_i:(x_i,x_{-i})\mapsto f_i(x_i,x_{-i})\in \mb{R}$.  Furthermore, each
$X_i$ can be finite-dimensional smooth manifolds or
infinite-dimensional Banach manifolds. Each player's cost function $f_i$ is
assumed to be sufficiently smooth. 

A two-player zero-sum game is characterized by a cost function $f\in C^r(X,\mb{R})$ in the sense that the first player aims to minimize $f$ with respect to $x_1$ and the second player aims to maximize $f$ with respect to $x_2$---that is, $f_1\equiv f$ and $\f_2\equiv -f$.
Hence, given a function $f$, we denote a two-player zero-sum game by $(f,-f)$ where $f\in C^r(X,\mb{R})$.

As is common in the study of games, we adopt the Nash equilibrium concept to
characterize the interaction between agents.
\begin{definition}
  \label{def:SLNE}
  A strategy $x=(\pxone{1}, \pxone{2})\in X$ is a {local Nash equilibrium}
  for the game $(f_1,f_2)=(\f, -\f)$ if for each $i\in\mc{I}$ there exists
  an open set $W_i\subset X_i$ such
  that $\pxone{i}\in W_i$ and %, $\pt_2\in W_2$, %for all $p'\in W_1\bs\{p\}$,
  \[f_i(x_i,x_{-i})\leq f_i(x_i',x_{-i}), \ \ \forall\ \pxone{i'}\in
  W_i\bs\{\pxone{i}\}.\]
%  \begin{equation}
   %   $\f_i(\pxone{1}, \ldots,\pxone{i},\ldots, \pxone{n})\leq \f_i(\pxone{1}, \ldots,
   %   \pxone{i'},\ldots, \pxone{n})$, %\ \ \forall \ \pt_i'\in W_i\bs\{\pt_i\}.
 %   \label{eq:ucondLN}
 % \end{equation}
    If the above inequalities are strict, then we say
    $(\pxone{1},x_2)$ is a {strict local Nash equilibrium}.
    If $W_i=X_i$ for each $i$, then $(\pxone{1},x_2)$ is a {global Nash
  equilibrium}. %\hfill\ensuremath{\blacksquare}
\end{definition}


In~\cite{ratliff:2013aa} and subsequent works~\cite{ratliff:2014aa,ratliff:2016aa}, a refinement of the local Nash equilibrium concept known as a
\emph{differential Nash equilibrium} was introduced. This refinement
characterizes local Nash in terms of first- and second-order conditions on
player cost functions, and even in the more general non-convex setting, a
differential Nash equilibrium was shown to be well-defined and independent of
the choice of coordinates on $X$. Moreover, for general sum games, differential Nash were shown to be
generic and structurally stable in $n$-player games. 
%; the
%extension of the later result 
%to $n$-player settings is fairly straightforward 
%and we present it in Section~\ref{sec:genericity}.

%We utilize the characterization of Nash equilibria provided
%in~\cite{ratliff:2016aa}. 
%Critical points for the game can be characterized by the so-called
%differential game form.
%\begin{definition} 
Towards defining the differential Nash concept, we introduce the following
mathematical object. A \emph{differential game form} is a differential 1-form $\omega: X\rar T^\ast X$ defined by
\[\textstyle\omega=\psi_{X_1}\circ d\f-\psi_{X_2}\circ d\f\]
    where $\psi_{X_i}$ are the natural bundle maps 
    %defined in \eqref{eq:bundles}
    $\psi_{X_1}: T^\ast X\rar T^\ast X$
    that annihilate those components of the co-vector field $d\f$
    corresponding to $X_1$ and analogously for $\psi_{X_2}$.
%\end{definition}
    Note that when each $X_i$ is a finite dimensional manifold of dimensions $m_i$
(e.g., Euclidean space $\mb{R}^{m_i}$), then the differential game form has the 
coordinate representation,
%\[\textstyle\omega_\psi=\sum_{j=1}^{m_1}\]
\[ 
  \textstyle  \omega_\psi=\sum_{j=1}^{m_1}\frac{\partial( \f\circ
\psi^{-1})}{\partial y_1^j}dy_1^j+\sum_{j=1}^{m_2}\frac{\partial( -\f\circ
\psi^{-1})}{\partial y_2^j}dy_2^j,\]
for product chart $(U,\psi)$ in $X$ at $x=(x_1,\ldots, x_n)$ with local
coordinates $(y_1^1, \ldots, y_{1}^{m_1}, y_2^1, \ldots, y_2^{m_2})$ and
where $U=U_1\times U_2$ and $\psi=\psi_1\times \psi_2$.
The differential game form captures a differential view of the
strategic interaction between the players. Note that each player's cost
function depends on its own choice variable as well as all the other
players’ choice variables. However, each player can only affect their
payoff by adjusting their own strategy.
%\bigtimes_{i=1}^n\psi_i

Critical points for the game can be characterized by the differential game form.
\begin{definition}
   A point $x\in X$ is said to be a {critical point} for the game if
    $\omega(x)=0$. 
    \label{def:criticalpt} 
\end{definition}
   In the single agent case (i.e., optimization of a single cost function),  critical points can be further classified as
    local minima, local maxima, or saddles by
    looking at second-order conditions. 
    %For instance, consider a single
    %agent with objective function
    %$f:X\rar\mb{R}$. Then a critical point $x$ is (i) a \emph{local minimum} if there
    %exists a neighborhood $U\subset X$ of $x$ such that
    %$f(x)\leq f(x')$ for all $x'\in U$, (ii) a \emph{local maximum} if there
    %exists a neighborhood $U\subset X$ of $x$ such that $f(x)\geq f(x')$, and
    %(iii) a \emph{saddle point} if for all neighborhoods $U\subset X$ of $x$, there are
    %$x_1,x_2\in U$ such that $f(x_1)\leq f(x)\leq f(x_2)$. 
%or, equivalently, $g(x^\ast)=x^\ast$.
    Analogous concepts exist for continuous games.
%As shown in~\cite{ratliff:2016aa}, if $x$ is a local Nash equilibrium for a cost
%minimization (respectively, utility maximization) game $(f_1,\ldots, f_n)$, then 
%  $\omega(\pt)=0$ and
%  $\D_{i}^2f_i(\pt)$ is positive semi-definite (respectively, negative semi-definite) for each
%  $i\in\mathcal{I}$.
\begin{proposition}[Proposition~2~\cite{ratliff:2013aa}]
    If $x\in X$ is a local Nash equilibrium for $(f_1,f_2)=(f,-f)$, then $\omega(x)=0$ and
    $D_{i}^2f_i(x)\geq 0$ for all $i\in \mc{I}$.
    \label{prop:necessary}
\end{proposition}
  %On the other hand, if $x$ is a local Nash equilibrium for a
  %utility maximization game $(f_1,\ldots, f_n)$, then 
  %$\omega(\pt)=0$ and
  %$\D_{ii}^2f_i(\pt)$ is negative semi-definite for each
  %$i\in\mathcal{I}$. 
  These are necessary conditions for a local Nash
  equilibrium. 
  %We will define a saddle point for the game 
%  Points $x=(\pxone{1},\ldots, \pxone{n})\in X_1\times \cdots \times X_n$ such that
% $\omega(x)=0$ are termed critical points of the game. 
There are also sufficient conditions for Nash equilibria. 
  Such sufficient conditions define differential Nash
  equilibria~\cite{ratliff:2016aa, ratliff:2014aa}.
  \begin{definition}
  \label{def:DNE}
  A strategy $x\in X$ is a {differential Nash equilibrium}
  for $(f_1,f_2)=(f,-f)$ if $\omega(\pt)=0$  and  $\D^2_{i}\f_i(x)$ is
  positive--definite for each $i\in\mc{I}$. 
  %\hfill\ensuremath{\blacksquare}
\end{definition}
Differential Nash need not be isolated. However, if
 $d\omega(x)$ is
non-degenerate for $x$ a differential Nash, where
$d\omega=d(\psi_{X_1}\circ d\f)-d(\psi_{X_2}\circ d\f),$
then $x$ is an \emph{isolated strict local Nash equilibrium}. Intrinsically,
$d\omega\in T_2^0(X)$ is a tensor field; at a point $x$ where $\omega(x)=0$, it
determines a bilinear form constructed from the uniquely determined continuous, symmetric, bilinear forms
$\{d^2f_i(x)\}_{i=1}^n$. 
%As shown in~\cite{ratliff:2016aa} via the simple example
%$\f_i(\pxone{i},\pxone{-i})=\frac{1}{2}x_i^2-x_ix_{-i}$,
%the conditions for differential Nash equilibria are not sufficient to guarantee that an equilibrium is isolated.
%However, for a differential Nash equilibrium $x$, . 
We use the notation
$D\omega$ to denote the bilinear map induced by $d\omega$ which is composed of
the partial derivatives of components of $\omega$. For example, consider a
two-player, zero-sum 
game $(\f_1,\f_2)=(f,-f)$. Then, via a slight abuse of notation, the matrix
representation of this bilinear map is given by
\[D\omega(x)=\bmat{D_{1}^2\f(x)  & D_{12}\f(x)\\  -D_{12}^T\f(x)  &
-D_{2}^2\f(x)}.\]

%\begin{definition}
%    We define a {saddle point} for the game $(f_1,\ldots, %f_n)$ to be a
%  critical point $x$ such that $D\omega(x)$ is indefinite.
%\end{definition}
% A saddle point such that
%$D\omega(x)$ has
%eigenvalues with $\text{Re}(\lambda_i)<0$, $i=1, \ldots, n_1$ %and
%$\text{Re}(\lambda_j)>0$, $j=1, \ldots, n_2$ with $m=n_1+n_2$ %and $n_1, n_2\neq
%0$ is a \emph{strict saddle point} or \emph{linearly unstable %critical point}---we
%use these terms interchangeably.

The following definitions are pertinent to our study of genericity and
structural stability of differential Nash equilibria; there are analogous
concepts in dynamical systems~\cite{broer:2010aa}.
    \begin{definition}
        A critical point $x$ is
    {non-degenerate} if $\det(D\omega(x))\neq 0$ (i.e.~$x$ is isolated).
    \label{def:nondegen}
    \end{definition}
    Non-degenerate differential Nash are strictly
    isolated local Nash equilibria~\cite[Theorem~2]{ratliff:2016aa}.
    \begin{definition}
        A critical point $x$ is
    {hyperbolic} if $D\omega(x)$ has no eigenvalues with zero real part.
    \label{def:hyperbolic}
    \end{definition}
All hyperbolic critical points are non-degenerate, but not all non-degenerate
critical points are hyperbolic. Hyperbolic critical points are of particular importance from the point of view of convergence, were they have local guarantees of exponential stability or instability \cite{sastry:1999ab}. We note that even in the more general manifold
setting, these definitions are invariant with respect to the coordinate
chart~\cite{ratliff:2016aa, broer:2010aa}.









%
%A critical point is
%    \emph{non-degenerate} if $\det(D\omega(x))\neq 0$ %(i.e.~$x$ is isolated).






==> [2019 CDC] Zero Sum Genericity (1)/intro.tex <==
\section{Introduction}
\label{sec:intro}

With machine learning algorithms increasingly being placed in more complex, real world settings, there has been a renewed interest in continuous games~\cite{ mertikopoulos:2019aa,zhang:2010aa, mazumdar:2018aa}, and particularly zero-sum continuous games~\cite{mazumdar:2019aa, daskalakis:2018aa, goodfellow:2014aa, jin:2019aa}. 
Adversarial learning~\cite{daskalakis:2017aa,mertikopoulos:2018aa}, robust reinforcement learning~\cite{li:2019aa, pinto:2017aa}, and generative adversarial networks~\cite{goodfellow:2014aa} all make use of zero-sum games played on highly non-convex functions to achieve remarkable results. 

Though progress is being made, a theoretical understanding of the equilibria of such games is lacking. 
In particular, many of the approaches to learning equilibria in these machine learning applications are gradient-based.
For instance, consider an adversarial learning setting where the goal is to learn a model or network by optimizing a function $f\in C^r(\Theta\times W,\mb{R})$ over $\theta\in \Theta$ where $w\in W$ is chosen by an adversary. A general approach to this problem is to study the coupled learning dynamics that arise when  one \emph{player} is descending $f$ and the other is ascending it---e.g.,
\begin{align*}
   \bmat{ \theta^+\\ w^+}=\bmat{\theta-\gamma D_\theta f(\theta,w)\\
w+\eta D_w f(\theta,w)}.
\end{align*}

%For instance, if the objective is to optimize some non-convex function $f:\Theta\times %W\rar\mb{R}$ over $\theta\in \Theta$ and where %
%
Most convergence analysis depends on an assumption of \emph{local convexity in the game space} around an equilibrium---that is, nearby Nash equilibria the Jacobian of the gradient-based learning rule is assumed to be locally positive definite. 
Indeed, with respect to the above example, in consideration of the limiting dynamics
 $\dot{x}=-\omega(x)$ where $x=(\theta, w)$ and $\omega(x)=(D_\theta f(x), -D_wf(x))$,
many of the convergence guarantees in this setting proceed under the assumption that around critical points, the Jacobian 
\[J(\theta, w)=\bmat{D_{\theta}^2f(\theta,w) & D_{\theta w}f(\theta,w)\\ -D_{w \theta}f(\theta,w) & -D_w^2f(\theta, w)}\]
is positive definite---i.e., there is some notion of \emph{local convexity in the game space}.
Given the structural assumptions often invoked in the analysis of these learning approaches, two questions naturally arise: 
\begin{itemize}
    \item  Is this a `robust' assumption in the sense of \emph{structural stability}---i.e., does the property persist under smooth perturbations to the game?;
    \item Is this assumption satisfied for `almost all zero-sum games' in the sense of \emph{genericity}?
\end{itemize}
Building on the work in~\cite{ratliff:2013aa, ratliff:2014aa, ratliff:2016aa}, this paper addresses these two questions. 

Towards this end, we leverage a refinement of the local Nash equilibrium concept that defines an equilibrium in terms of the first- and second-order optimality conditions for each player holding all other players fixed.   This refinement has implicitly in its definition this notion of local convexity in the game space; it also has a structure that is particularly amenable to computation and which can be exploited in learning since it is characterized in terms of local information. Efforts to show this refinement is both structurally stable and generic aid in justifying its broad use.

\subsection{Contributions}
The contributions are summarized as follows: 

a. We prove that differential Nash equilibria---a refinement of local Nash equilibria defined in terms of first- and second-order conditions which characterize local optimality for players---are generic amongst local Nash equilibria in continuous zero-sum games (Theorem~\ref{thm:main}). This implies that almost all zero-sum games played on continuous functions admit local Nash equilibria that are strict and isolated.

b. Exploiting the underlying structure of zero-sum game---i.e., the game is defined in terms of a single sufficiently smooth cost function---we show that all differential Nash equilibria are hyperbolic (Proposition~\ref{prop:hyperbolic}), meaning they are locally exponentially attracting for gradient-play. Combining this fact with the above, we also show that local Nash equilibria are generically hyperbolic (Corollary~\ref{cor:hyperbolic}).

c. We prove that zero-sum games are structurally stable (Theorem~\ref{thm:ss_zsg}); that is, the structure of the game---and hence, its equilibria---is robust to smooth perturbations within the space of zero-sum games.

 
 In~\cite{ratliff:2013aa, ratliff:2014aa, ratliff:2016aa}, similar results to a.~and c.~were shown for the larger class of general-sum continuous games. Yet, the set of zero-sum games is of zero measure in the space of general-sum continuous games, and hence, the results of this paper are not a direct implication of those results.
 Further, b.~is a much stronger statement than the genericity result in~\cite{ratliff:2014aa}. In particular,~\cite{ratliff:2014aa} shows that non-degenerate differential Nash equilibria are generic amongst local Nash equilibria. We, on the other hand, show that in the class of zero-sum games, \emph{all differential Nash equilibria are non-degenerate, and moreover, hyperbolic}. The latter is a particularly strong result, achievable due to the specific structure of the zero-sum game. Indeed, two-player zero-sum continuous games are defined completely in terms of a single sufficiently smooth function---i.e., given $f\in C^r(X,\mb{R})$, the corresponding zero-sum game is $(f,-f)$.
 %$\{(f,-f)|\ f\in C^r(X, \mb{R})\}$ is defined 
%
% 
% we go beyond the results in 
% Exploiting the structure of zero-sum games, we go beyond the results in~\cite{ratliff:2014aa} by showing that all differential Nash equilibria are in fact hyperbolic,   

Moreover, the work in this paper focuses on a class of games of particular import to the machine learning and robust control communities, where many recent works have made the assumption of hyperbolicity of local Nash equilibria without a thorough understanding of whether or not such an assumption is restrictive (see e.g. \cite{Daskalakis2018TheLP,balduzzi:2018aa,PotentialGameBanditFeed,VariationalGAN,jin:2019aa}). The results in this paper show that this assumption simply \emph{rules out a measure zero set of zero-sum games}. 
%We provide simple illustrative examples that reinforce the theoretical ideas.

%\subsection{Organization}
%The organization of the remainder of the paper is a reflection of the fact that it is a short technical note. Section~\ref{sec:setup} contains both mathematical and game-theoretic preliminaries; additional differential geometry preliminaries are provided in Appendix~\ref{app:prelims}. The main results of the paper are contained in Section~\ref{sec:thm}. Section~\ref{subsec:genericity} includes \emph{(i)} a statement and proof of the claim that differential Nash are generic amongst local Nash in the class of two-player, zero-sum continuous games; and, \emph{(ii)} a proof that all differential Nash are in fact non-degenerate and all non-degenerate critical points are hyperbolic. This implies that hyperbolic differential Nash are generic amongst local Nash in zero-sum games. Section~\ref{subsec:structuralstability} contains a statement and proof of the fact that differential Nash are robust to smooth perturbations in the game structure. Section~\ref{sec:num_ex} contains examples intended to illustrate the theory and provide the reader with intuition. Finally, Section~\ref{sec:conclusion} contains discussion and concluding remarks.

==> [2019 CDC] Zero Sum Genericity (1)/math_prelims.tex <==
\subsection{Mathematical Preliminaries}

In order to prove genericity of non-degenerate differential Nash, we now introduce the necessary mathematical preliminaries.

Consider smooth manifolds $X$ and $Y$ of dimension $n_x$ and $n_y$ respectively.
An \emph{$k$--jet} from $X$ to $Y$ is an equivalence class $[x,\f,U]_k$ of
triples $(x,\f,U)$ where $U\subset X$ is an open set, $x\in U$, and $f:U\rar Y$
is a $C^k$ map. The equivalence relation satisfies $[x,\f,U]_k=[y,g,V]_k$ if
$x=y$ and in some pair of charts adapted to $\f$ at $x$, $\f$
and $g$ have the same derivatives up to order $k$. We use the notation
$[x,\f,U]_k=j^k\f(x)$ to denote the $k$--jet of $f$ at $x$. The set of all
$k$--jets from $X$ to $Y$ is denoted by $J^k(X,Y)$. The jet bundle $J^k(X, Y)$
is a smooth manifold (see \cite{Hirsch:1976la} Chapter 2 for the construction).
For each $C^k$ map $f:X\rar Y$ we define a map $j^kf:X\rar J^k(X, Y)$ by $x\mapsto j^kf(x)$ and refer to it as the \emph{$k$--jet extension}. 

\begin{definition}
Let $X$, $Y$ be smooth manifolds and $f:X\rar Y$ be a smooth mapping. Let $Z$ be
a smooth submanifold of $Y$ and $p$ a point in $X$. Then \emph{$f$ intersects
$Z$ transversally at $p$} (denoted $f\pitchfork Z$ at $p$) if either $f(p)\notin
Z$ or $f(p)\in Z$ and $T_{f(p)} Y=T_{f(p)}Z + (f_\ast)_p(T_pX)$.
%\begin{enumerate}
%  \item $f(p)\notin Z$, or
%  \item $f(p)\in Z$ and $T_{f(p)} N=T_{f(p)}Z + (f_\ast)_p(T_pM)$.
%\end{enumerate}
\end{definition}

For $1\leq k<s\leq \infty$ consider the jet map 
%\begin{equation}
  $j^k:C^s(X, Y)\rar C^{s-k}(X, J^k(X, Y))$
%  \label{eq:jetmap}
%\end{equation}
and let $Z\subset J^k(X, Y)$ be a submanifold. 
Define
\begin{equation}
  \trans^s(X, Y; j^k, Z)=\{ h\in C^s(X, Y)|\ j^kh \pitchfork Z\}.
  \label{eq:jettrans}
\end{equation}
A subset of a topological space $X$ is \emph{residual} if it contains the intersection of countably many open--dense sets. We say a property is \emph{generic} if the set of all points of $X$ which possess this property is residual~\cite{broer:2010aa}. 
%\sam{Need def of strong topology.}

%We now introduce the \emph{strong topology} on $C^k(M, N)$. Let $\Phi=\{(U_i, \vphi_i)\}_{i\in I}$ be a locally finite set of charts on $M$ for some index set $I$. Let $K=\{K_i\}_{i\in I}$ be a family of compact subsets of $M$ such that $K_i\subset U_i$. Similarly, let $\Psi=\{(V_i, \psi_i)\}_{i\in I}$ be a family of charts on $N$ and $\{\vep_i\}_{i\in I}$ a family of positive numbers. Then, if $f\in C^k(M, N)$ takes each $K_i$ into $V_i$, then the set that contains all maps $g\in C^k(M, N)$ such that for all $i\in I$, $g(K_i)\subset V_i$ and 
%\begin{equation}
%  \|D^r(\psi_i\circ f\circ \vphi_i^{-1})(x)-D^r(\psi_i\circ g\circ \vphi_i^{-1})(x)\|\leq \vep_i
%  \label{eq:strongtop}
%\end{equation}
%for all $x\in \vphi_i(K_i)$, $r=0, \ldots, k$ is a \emph{strong basic neighborhood}. The strong topology has all possible sets of this form as its base.

%The following results will be used to prove genericity of non--degenerate differential Nash equilibria.

%{\it Theorem 2.8 in~\cite{Hirsch:1976la} \emph{(Jet Transversality)}}
\begin{theorem}(Jet Transversality Theorem, Chap.~2 \cite{Hirsch:1976la}).
  Let $X$, $Y$ be $C^\infty$ manifolds without boundary, and let $Z\subset
  J^k(X, Y)$ be a $C^\infty$ submanifold. Suppose that $1\leq k<s\leq \infty$.
  Then, $\trans^s(X, Y; j^k, Z)$ is residual and thus dense in $C^s(X, Y)$ endowed with the strong topology, and open if $Z$ is closed. 
\label{thm:jettrans}
\end{theorem}
\begin{proposition}
  \label{prop:intersect}
  (Chap.~II.4, Proposition 4.2~\cite{golubitsky:1973aa}). Let $X,Y$ be smooth
  manifolds and $Z\subset Y$ a submanifold. Suppose that $\dim X< \codim Z$. Let
  $f:X\rar Y$ be smooth and suppose that $f\pitchfork Z$. Then, $f(X)\cap Z=\emptyset$.
\end{proposition}
%In Section~\ref{sec:genericity}, we use an argument based on the co--dimension of the set of functions which do not have the properties we desire Theorem~\ref{thm:jettrans} allos
%The concepts introduced in this section are very important for the development of our main results. 

%The definition of residual set, and hence genericity, implies a notion of \emph{almost all} which will be necessary for showing that local Nash equilibria are generically non-degenerate differential Nash equilibria. 
%The latter have nice properties; they are isolated, structurally stable as we will see in Section~\ref{sec:stable}, and hence computable.

The Jet Transversality Theorem and Proposition~\ref{prop:intersect} can be used to show a subset of a jet bundle having a particular set of desired properties is generic. 
Indeed, consider the jet bundle $J^k(X, Y)$ and recall that it is a manifold
that contains jets $j^kf:X\rar J^k(X, Y)$ as its elements where $f\in C^k(X,
Y)$. Let $Z\subset J^k(X, Y)$ be the submanifold of the jet bundle that \emph{does not} possess the desired properties. 
If $\dim X<\codim\ Z$, then for a generic function $f\in C^k(X, Y)$ the image of the $k$--jet extension is disjoint from $Z$ implying that there is an open--dense set of functions having the desired properties. 
It is exactly this approach we use to show the genericity of non-degenerate differential Nash equilibria of zero-sum continuous games.


==> [2019 CDC] Zero Sum Genericity (1)/related_work.tex <==
\section{Related Work}
\label{sec:related_work}



==> [2019 CDC] Zero Sum Genericity (1)/theorems.tex <==
\section{Useful Theorems}

In order to prove genericity of non-degenerate differential Nash, we need some 
mathematical prelimiaries.

\subsection{Preliminaries}
Consider smooth manifolds $X$ and $Y$ of dimension $n_x$ and $n_y$ respectively.
An \emph{$k$--jet} from $X$ to $Y$ is an equivalence class $[x,\f,U]_k$ of
triples $(x,\f,U)$ where $U\subset X$ is an open set, $x\in U$, and $f:U\rar Y$
is a $C^k$ map. The equivalence relation satisfies $[x,\f,U]_k=[y,g,V]_k$ if
$x=y$ and in some (and hence any) pair of charts adapted to $\f$ at $x$, $\f$
and $g$ have the same derivatives up to order $k$. We use the notation
$[x,\f,U]_k=j^k\f(x)$ to denote the $k$--jet of $f$ at $x$. The set of all
$k$--jets from $X$ to $Y$ is denoted by $J^k(X,Y)$. The jet bundle $J^k(X, Y)$
is a smooth manifold (see \cite{Hirsch:1976la} Chapter 2 for the construction).
For each $C^k$ map $f:X\rar Y$ we define a map $j^kf:X\rar J^k(X, Y)$ by $x\mapsto j^kf(x)$ and refer to it as the \emph{$k$--jet extension}. 
%Suppose that $(U, \vphi)$ and $(V, \psi)$ are charts on $M$ and $N$ respectively. Let $\tilde{f}\in C^k(U, \mb{R}^n)$ Then $k$--jet of $\tilde{f}$ at $x\in U$
\begin{definition}
Let $X$, $Y$ be smooth manifolds and $f:X\rar Y$ be a smooth mapping. Let $Z$ be
a smooth submanifold of $Y$ and $p$ a point in $X$. Then \emph{$f$ intersects
$Z$ transversally at $p$} (denoted $f\pitchfork Z$ at $p$) if either $f(p)\notin
Z$ or $f(p)\in Z$ and $T_{f(p)} Y=T_{f(p)}Z + (f_\ast)_p(T_pX)$.
%\begin{enumerate}
%  \item $f(p)\notin Z$, or
%  \item $f(p)\in Z$ and $T_{f(p)} N=T_{f(p)}Z + (f_\ast)_p(T_pM)$.
%\end{enumerate}
\end{definition}

For $1\leq k<s\leq \infty$ consider the jet map 
%\begin{equation}
  $j^k:C^s(X, Y)\rar C^{s-k}(X, J^k(X, Y))$
%  \label{eq:jetmap}
%\end{equation}
and let $Z\subset J^k(X, Y)$ be a submanifold. 
Define
\begin{equation}
  \trans^s(X, Y; j^k, Z)=\{ h\in C^s(X, Y)|\ j^kh \pitchfork Z\}.
  \label{eq:jettrans}
\end{equation}
A subset of a topological space $X$ is \emph{residual} if it contains the intersection of countably many open--dense sets. We say a property is \emph{generic} if the set of all points of $X$ which possess this property is residual~\cite{broer:2010aa}. 
%\sam{Need def of strong topology.}

%We now introduce the \emph{strong topology} on $C^k(M, N)$. Let $\Phi=\{(U_i, \vphi_i)\}_{i\in I}$ be a locally finite set of charts on $M$ for some index set $I$. Let $K=\{K_i\}_{i\in I}$ be a family of compact subsets of $M$ such that $K_i\subset U_i$. Similarly, let $\Psi=\{(V_i, \psi_i)\}_{i\in I}$ be a family of charts on $N$ and $\{\vep_i\}_{i\in I}$ a family of positive numbers. Then, if $f\in C^k(M, N)$ takes each $K_i$ into $V_i$, then the set that contains all maps $g\in C^k(M, N)$ such that for all $i\in I$, $g(K_i)\subset V_i$ and 
%\begin{equation}
%  \|D^r(\psi_i\circ f\circ \vphi_i^{-1})(x)-D^r(\psi_i\circ g\circ \vphi_i^{-1})(x)\|\leq \vep_i
%  \label{eq:strongtop}
%\end{equation}
%for all $x\in \vphi_i(K_i)$, $r=0, \ldots, k$ is a \emph{strong basic neighborhood}. The strong topology has all possible sets of this form as its base.

%The following results will be used to prove genericity of non--degenerate differential Nash equilibria.

%{\it Theorem 2.8 in~\cite{Hirsch:1976la} \emph{(Jet Transversality)}}
\begin{theorem}(Jet Transversality Theorem, Chapter 2 of \cite{Hirsch:1976la}).
  Let $X$, $Y$ be $C^\infty$ manifolds without boundary, and let $Z\subset
  J^k(X, Y)$ be a $C^\infty$ submanifold. Suppose that $1\leq k<s\leq \infty$.
  Then, $\trans^s(X, Y; j^k, Z)$ is residual and thus dense in $C^s(X, Y)$ endowed with the strong topology, and open if $Z$ is closed. 
\label{thm:jettrans}
\end{theorem}
\begin{proposition}
  \label{prop:intersect}
  (Chapter II.4, Proposition 4.2~\cite{golubitsky:1973aa}). Let $X,Y$ be smooth
  manifolds and $Z\subset Y$ a submanifold. Suppose that $\dim X< \codim Z$. Let
  $f:X\rar Y$ be smooth and suppose that $f\pitchfork Z$. Then, $f(X)\cap Z=\emptyset$.
\end{proposition}
%In Section~\ref{sec:genericity}, we use an argument based on the co--dimension of the set of functions which do not have the properties we desire Theorem~\ref{thm:jettrans} allos
%The concepts introduced in this section are very important for the development of our main results. 

%The definition of residual set, and hence genericity, implies a notion of \emph{almost all} which will be necessary for showing that local Nash equilibria are generically non-degenerate differential Nash equilibria. 
%The latter have nice properties; they are isolated, structurally stable as we will see in Section~\ref{sec:stable}, and hence computable.

The Jet Transversality Theorem and Proposition~\ref{prop:intersect} can be used to show a subset of a jet bundle having a particular set of desired properties is generic. 
Indeed, consider the jet bundle $J^k(X, Y)$ and recall that it is a manifold
that contains jets $j^kf:X\rar J^k(X, Y)$ as its elements where $f\in C^k(X,
Y)$. Let $Z\subset J^k(X, Y)$ be the submanifold of the jet bundle that \emph{does not} possess the desired properties. 
If $\dim X<\codim\ Z$, then for a generic function $f\in C^k(X, Y)$ the image of the $k$--jet extension is disjoint from $Z$ implying that there is an open--dense set of functions having the desired properties. 
%We will use this argument in Section~\ref{sec:generic} to show that non--degenerate differential Nash equilibria are generic among local Nash equilibria. 


% \subsection{Hyperbolic Critical Points}
% \begin{theorem}
%     Critical points of vector fields are generically hyperbolic.     \label{thm:hyperbolic}
% \end{theorem}
% The above theorem is standard in dynamical systems theory. This implies that
% critical points of $\dot{x}=-\omega(x)$ for both general and zero-sum games are
% generically hyperbolic.
% \begin{proof}
%     Let $\mc{B}$ be the subset of matrices in which have at least one eigenvalue
%     on the imaginary axis. This is a semi-algebraic set. Indeed, 
%     \[\mc{B}^\ast=\{(A, t)|\ \det(A-itI)=0\}\]
%     is by definition an algebraic (hence semi-algebraic) subset of
%     $\mb{R}^{m\times m}\times\mb{R}$. Note that $\mc{B}$ is the projection of
%     $\mc{B}^\ast$ on to $\mb{R}^{m\times m}$. Since the image of a semi-algebraic set
%     under an algebraic map is at least semi-algebraic, then $\mc{B}$ is also
%     semi-algebraic. Since $\mc{B}$ has no interior points, it is the union of
%     submanifolds of co-dimension greater than or equal to one. 

%     Applying Theorem~\ref{thm:jettrans} for $1$-jet extensions to vector fields
%     as maps from $\mb{R}^m$ to itself. That is, we are considering a vector
%     field as a map taking $\mb{R}^m$ to $\mb{R}^m$ and considering its $1$-jet
%     extensions which are denoted by $J^1(\mb{R}^m, \mb{R}^m)$. Note that $J^1(\mb{R}^m, \mb{R}^m)$ can
%     be canonically identified with $\mb{R}^{m}\times \mb{R}^m\times
%     \mb{R}^{m\times m}$ so that the $1$-jet of $V$ at $x$ is identified with
%     $(x, V(x), DV(x))$. 

%     Consider $G_1=\mb{R}^m\times \{0\}\times\mc{B}$. From above, $G_1$ is the
%     union of submanifolds of codimensions greater than or equal to $m+1$. Hence,
%     $j^1V$ from $\mb{R}^m$ to $\mb{R}^m$ is transversal with respect to $G_1$ if
%     and only if the image of $j^1V$ is disjoint from $G_1$. The Jet
%     Transversality Theorem implies that for generic $C^r$ vector fields $V$ with
%     $r\geq 2$, the image of the $1$-jet extension $J^1(V)$ is disjoint from
%     $\mc{B}$ which gives the result that critical points being hyperbolic is a
%     generic property.
    
% \end{proof}





==> [2019 CDC] Zero Sum Genericity (1)/theoretical_results.tex <==
\section{Theoretical Results}
\label{sec:thm}
In this section, we specialize the results in~\cite{ratliff:2013aa} and \cite{ratliff:2016aa} on genericity and structural stability of differential Nash equilibria to the class of zero-sum games. 
\subsection{Genericity}
\label{subsec:genericity}
To develop the proof that local Nash equilibria of zero-sum games are generically non-degenerate differential Nash equilibria, we leverage the fact that it is a generic property of sufficiently smooth functions that all critical points are non-degenerate. 
\begin{lemma}[{\cite[Chapter~1]{broer:2010aa}}]
    For $C^r$ functions, $r\geq 2$ on $\mb{R}^n$, or on a manifold, it is a
    generic property that all the critical points are non-degenerate.
    \label{lem:generic}
\end{lemma}

The above lemma implies that
for a generic function $f\in C^r(X,\mb{R})$ on an $m$--dimensional manifold $X$, the Hessian
\[H(x)=\bmat{D_{1}^2f(x) & \cdots & D_{1m}f(x)\\
    \vdots &\ddots & \vdots\\
D_{m1}f(x)& \cdots & D_{m}^2f(x)}\]
is non-degenerate at critical points---that is, $\det(H(x))\neq 0$. 
\begin{lemma}
    Consider $f\in C^r(X, \mb{R})$ and the zero-sum game $(f,-f)$. For any critical point $x\in X$ (i.e., $x\in\{x\in X|\ \omega(x)=0\}$), 
    $\det(H(x))\neq 0\Longleftrightarrow\det(D\omega(x))\neq 0.$
    \label{lem:equiv}
\end{lemma}

\begin{proof}
 Before proceeding  we note that in the case that $X$ is a smooth manifold, the stationarity of critical points and definiteness of $H$ and $D\omega$ are  coordinate-invariant properties and hence, independent of coordinate chart~\cite{ratliff:2013aa, ratliff:2014aa, ratliff:2016aa, broer:2010aa}. Thus, to shorten the presentation of proofs, we simply treat the Euclidean case here; showing the more general case simply requires selecting a coordinate chart defined on a neighborhood of the differential Nash, showing the results with respect to this chart, and then invoking coordinate invariance.
 
 Let $x=(x_1,x_2)$ where $X=X_1\times X_2$ and $X_i$ is $m_i$--dimensional. Note that $H(x)$ is equal to $D\omega(x)$ with the last $m_2$ rows scaled
    each by $-1$. Indeed,
    \[D\omega(x)=\bmat{D_1^2f(x) & D_{12}f(x)\\ 
    -D_{12}^Tf(x) & -D_2^2f(x)}\]
    where $D_i^2f(x)$ is $m_i\times m_i$ dimensional for each $i\in\{1,2\}$ and $D_{12}f(x)$ is $m_1\times m_2$ dimensional.
    %\bmat{D_{1}^2f(x) & \cdots & D_{1m}f(x)\\
    %\vdots &\ddots & \vdots\\
    %D_{m_11}f(x) & \cdots & D_{m_1m}f(x)\\
    %-D_{m_1+11}f(x) & \cdots & -D_{m_1+1m}f(x)\\
    %   \vdots &\ddots & \vdots\\
%-D_{m1}f(x)& \cdots & -D_{m}^2f(x)}\]
Clearly, $D\omega(x)=PH(x)$ where $P=\text{blockdiag}(I_{m_1},-I_{m_2})$ with each $I_{m_i}$ the $m_i\times m_i$ identity matrix, so that
 %   Since the determinant of a matrix with rows that are scaled
 %   is just a scaling of the determinant, we have that
    $\det(H(x))=(-1)^{m_2}\det(D\omega(x))$.
    Hence, the result holds. 
\end{proof}

This equivalence between the non-degeneracy of the Hessian and the game Jacobian $D\omega$ allows us to lift the fact that non-degeneracy of critical points is a generic property to zero-sum games.
%are generic of non-degenerate critical points 
%    \begin{proof}
%This is obvious if $m=m_1+m_2=2$. Suppose now that $m>2$.   
% In particular, let $x_i\in X_i$ where $\dim(X_i)=m_i$.
%Now, consider any matrix
%\[M=\bmat{A & B\\  C& D}\]
%with $A\in \mb{R}^{m_1\times m_1}, B\in \mb{R}^{m_1\times m_2}, C\in
%\mb{R}^{m_2\times m_1}$, and $D\in \mb{R}^{m_2\times m_2}$. Then, wlog, if $D$
%is invertible then 
%\[\det(M)=\det(A-BD^{-1}C)\det(D)\]
%\begin{description}
%    \item[case 1.] Suppose $\det(D_{2}^2f(x))\neq 0$, then 
%\[\det(H(x))=\det(D_1^2f(x)-D_{12}f(x)(D_2^2f(x))^{-1}D_{21}f(x))\det(D_{2}^2f(x))\]
%and
%\[\det(D\omega(x))=\det(D_1^2f(x)-D_{12}f(x)(D_2^2f(x))^{-1}D_{21}f(x))\det(-D_{2}^2f(x))\]
%so that these are clearly non-zero when the other is.
%\item[case 2.] On the other hand, suppose
%$D_1^2f$ is non-degenerate. Then,
%\[\det(H(x))=\det(D_2^2f(x)-D_{21}f(x)(D_1^2f(x))^{-1}D_{12}f(x))\det(D_{1}^2f(x))\]
%and
%\[\det(D\omega(x))=\det(-D_2^2f(x)+D_{21}f(x)(D_1^2f(x))^{-1}D_{12}f(x))\det(D_{1}^2f(x))\]
%so again we have equivalence between $\det(H)\neq0$ and $\det(D\omega)\neq 0$.
%\item[case 3.] Suppose now both $\det(D_{i}^2f(x))=0$. We claim that either both
%    $H$ and $D\omega$ are degenerate or they are both not. Suppose not. That is,
%    WLOG
%    suppose that $\det(H(x))=0$ and $\det(D\omega(x))\neq 0$. 
%    \[H=\bmat{D_1^2f & D_{12}f\\ D_{21}f & D_{2}^2f}\]
%\[D\omega=\bmat{D_1^2f & D_{12}f\\ -D_{12}f^T & -D_{2}^2f}\]
%\textcolor{Red}{This has to be the case because
%    $\det(H(x))=(-1)^{k}\det(D\omega(x))$ where the $k$ determines a sign flip
%and is related to the number of choice variables}.
%\end{description}
%    \end{proof}

\begin{proposition}
Consider a two-player, zero-sum continuous game $(f,-f)$ defined for $f\in C^r(X,\mb{R})$ with $r\geq 2$. A differential Nash equilibrium is non-degenerate, and furthermore, it is hyperbolic. 
\label{prop:hyperbolic}
\end{proposition}
\begin{proof}
     It is enough to show that all differential Nash are hyperbolic since all hyperbolic equilibria correspond to a non-degenerate $D\omega$. Further, just as we noted in the proof of Lemma~\ref{lem:equiv}, stationarity, definiteness, and non-degeneracy are coordinate-invariant properties. Thus, we simply treat the Euclidean case here.
     %We first show that differential Nash equilibria in zero-sum games are hyperbolic equilibria. 
     
     By definition, at a differential Nash equilibrium $x$ of a zero-sum game, $\omega(x)=0$, $D^2_1f(x)> 0$, and $-D^2_2f(x)>0$. Further, in zero-sum games, $D^2_{12}f=(D^2_{21}f)^T$. Thus, the bilinear map $D\omega$, takes the form
\begin{align*}
    D\omega(x)&=\bmat{D^2_1f(x) & D_{12}f(x) \\ -D_{21}f(x) & -D^2_{2}f(x)}\\
    &= \bmat{D^2_1f(x) & D_{12}f(x) \\ -D_{12}^Tf(x)& -D^2_{2}f(x)}.
\end{align*}
    Let $(\lambda,v)$ be an eigenpair of $D\omega(x)$. The real part of $\lambda$, denoted $\mathrm{Re}(\lambda)$, can be written as
\begin{align*}
\textstyle\mathrm{Re}(\lambda)&=\textstyle\frac{1}{2}(\lambda +\bar \lambda)=\textstyle\frac{1}{2} (v^*D\omega^T(x)v+v^*D\omega(x)v)\\
&=\textstyle\frac{1}{2} v^*(D\omega^T(x)+D\omega(x))v\\
&=\frac{1}{2} v^*\bmat{D^2_1f(x) &0 \\ 0& -D^2_{2}f(x)}v>0
\end{align*}
where the last line follows from the positive definiteness of $\diag(D^2_1f(x),-D_2^2f(x))$
%\[ \bmat{D^2_1f(x) & 0 \\ 0& -D^2_{2}f(x)},\]
at a differential Nash equilibrium. Hence, $x$ is hyperbolic and, clearly, at this point $\det(D\omega(x))\neq 0$.
\end{proof}

The above proposition provides a strong result for the class of zero-sum games. In particular, simply due to the structure of $D\omega$, all differential Nash have the nice property of being hyperbolic, and hence, exponentially attracting under gradient-play dynamics---that is, $\dot{x}=-\omega(x)$ or its discrete time variant $x^+=x-\gamma \omega(x)$ for appropriately chosen stepsize $\gamma$. Note that numerous learning algorithms in machine learning applications of zero-sum games take this form~(see, e.g., \cite{goodfellow:2014aa, mazumdar:2018aa, mazumdar:2019aa}). 

\begin{theorem}
    For two-player, zero-sum continuous games, non-degenerate differential Nash are generic amongst
    local Nash equilibria. That is, given a generic $f\in C^r(X, \mb{R})$, all local
    Nash equilibria of the game $(f,-f)$ are (non-degenerate) differential Nash
    equilibria. 
    \label{thm:main}
\end{theorem}
\begin{proof}
    First, critical points of a function $f$ are those such that
    $(D_1f_1(x)\ D_2f_2(x))=0$ and hence they coincide with critical points of
    the zero-sum game---i.e., those points $x$ such that $\omega(x)=(D_1f(x),
    -D_2f(x))=0$. By Lemma~\ref{lem:equiv}, for any critical point $x$, $\det(H(x))=0$ if and
    only if $\det(D\omega(x))=0$. Hence, critical points of $f$ are
    non-degenerate if and only if critical points of the zero-sum game are
    non-degenerate. 

Consider a generic function $f$ and the
    corresponding zero-sum game $(f,-f)$. If $X$ is a smooth manifold, let $(U, \varphi)$ be a product chart on $X_1\times X_2$ that contains $x$. Suppose that $x$ is a local Nash
    equilibrium so that $\omega(x)=0$ and $D_1^2f(x)\geq 0$ and $-D_2^2f(x)\geq
    0$. By the above argument, since $f$ is generic and the critical points of
    $f$ coincide with those of the zero-sum game, $\det(D\omega(x))\neq 0$.   By Lemma~\ref{lem:generic}, critical points of a generic zero-sum
    game are non-degenerate. That is, there exists an open-dense set of
    functions $f$ in $C^r(X, \mb{R})$ such that critical points of the
    corresponding game are non-degenerate. 
    
    

%    \textcolor{Red}{Ok, so the part I am stuck at proving is that for smooth
%        functions $f$, $\det(D_{i}^2f(x))\neq 0$ is a generic property. This is
%    the argument using $G_2$ in my ACC paper which doesnt extend because it
%    would give us a open-dense set in the space $C^\infty(X, \mb{R}^2)$ and not
%    in $C^\infty(X, \mb{R})$.
%\newline\newline
%\textbf{attempt proof}: 
  Let $J^2(X, \mb{R})$ denote the second-order jet bundle containing $2$--jets $j^2f$ such that $f:X\rar \mb{R}$. Then, $J^2(X, \mb{R})$ is locally diffeomorphic to 
  \[\mb{R}^m\times \mb{R}\times \mb{R}^m\times \mb{R}^{\frac{m(m+1)}{2}}\]
  and the $2$--jet extension of $f$ at any point $x\in X$ in coordinates is given by
  \[(\varphi(x), (f\circ\varphi^{-1})(\varphi(x)), D^\varphi f(x), (D^\varphi)^2f(x))\]
  where $D^\varphi f=[D^\varphi_1f\ D^\varphi_2f]$ with $D^\varphi_j=[\partial (f\circ \varphi^{-1})/(\partial y_j^1)\ \cdots \ \partial (f\circ \varphi^{-1})/(\partial y_j^{m_i})]$ and similarly for $(D^\varphi)^2f$. Again, we note that the properties of interest (stationarity, definiteness, and non-degeneracy) are known to be coordinate invariant. 
  
  Consider a subset of $J^2(X, \mb{R})$ defined by 
\[\mc{D}=\mb{R}^m\times \mb{R}\times \{0_m\}\times Z(m_1)\times \mb{R}^{m_1\times
m_2}\times Z(m_2)\]
where $Z(m_i)$ is the subset of symmetric $m_i\times m_i$ matrices such that for
$A\in Z(m_i)$, $\det(A)=0$. Each $Z(m_i)$ is algebraic and has no interior
points; hence, we can use the Whitney stratification theorem~\cite[Chapter 1, Theorem 2.7]{gibson:1976ab} to get that each
$Z(m_i)$ is the union of submanifolds of co-dimension at least $1$. Hence $\mc{D}$
is the union of submanifolds and has co-dimension at least $m+2$. Applying the
Jet Transversality Theorem (Theorem~\ref{thm:jettrans}) and
Proposition~\ref{prop:intersect} yields an open-dense set of functions $f$ such
that when $\omega(x)=0$, $\det(D_i^2f(x))\neq 0$, for $i=1,2$.

Now, the intersection of two open-dense sets is open-dense so that we have an
open-dense set of functions $f$ in $C^r(X, \mb{R})$ such that when
$\omega(x)=0$, $\det(D_i^2f(x))\neq 0$ for each $i\in\{1,2\}$ and
$\det(D\omega(x))\neq 0$. 
This, in turn, implies that there is an open-dense set $\mc{F}$ of functions $f$ in
$C^r(X,\mb{R})$ such that for zero-sum games constructed from these
functions, local Nash equilibria are non-degenerate differential Nash
equilibria. Indeed, consider an $f\in \mc{F}$ in this set such that $x$ is a
local Nash equilibrium of $(f,-f)$. Then necessary conditions for Nash imply
that $\omega(x)=0$, $D_1^2f(x)\geq 0$ and $-D_2^2f(x)\geq 0$. However, since
$f\in \mc{F}$, $\det(D_1^2f(x))\neq 0$ and $\det(-D_2^2f(x))=(-1)^{m_2}\det(D_2^2f(x))\neq
0$. Hence, $x$ is a differential Nash equilibrium. Moreover, since $f\in
\mc{F}$, $\det(H(x))\neq 0$ which is equivalent to $\det(D\omega(x))\neq 0$ (by
Lemma~\ref{lem:equiv}). Thus, $x$ is a non-degenerate differential Nash. 
%$\mc{ZS}$
%}
%\hfill$\blacksquare$
\end{proof}

As shown in Proposition~\ref{prop:hyperbolic}, all differential Nash for zero-sum games are non-degenerate simply by the structure of $D\omega$. This further implies that local Nash equilibria are generically hyperbolic critical points, meaning there are no eigenvalues of $D\omega$ with zero real part.
\begin{corollary}
    Within the class of two-player zero-sum continuous games, local Nash equilibria are generically hyperbolic critical points.
    \label{cor:hyperbolic}
\end{corollary}
\begin{proof}
  Consider a two-player, zero-sum game $(f,-f)$ for some generic sufficiently smooth $f\in C^r(X, \mb{R})$. Then, by Theorem~\ref{thm:main}, a local Nash equilibria $x$ is a differential Nash equilibria. Moreover,  by Proposition~\ref{prop:hyperbolic}, $x$ is hyperbolic so that all eigenvalues of $D\omega(x)$ must have strictly positive real parts. This implies that all such points are hyperbolic critical points of the gradient dynamics $\dot{x}=-\omega(x)$. 
  %Invoking Theorem~\ref{thm:main} completes the proof. Indeed, Theorem~\ref{thm:main} gives us that for a generic function $f\in C^r(X,\mb{R})$, all the local Nash equilibria of the game $(f,-f)$ are (non-degenerate) differential Nash which hyperbolic by the above argument. 
\end{proof}

\subsection{Structural Stability}
\label{subsec:structuralstability}
Genericity gives a formal mathematical sense of 'almost all' for a certain property---in this case, non-degeneracy and further hyperbolic. In addition, we show that (non-degenerate) differential Nash are structurally stable, meaning that they persist under smooth perturbations within the class of zero-sum games.
\begin{theorem}
    For zero-sum games, differential Nash equilibria are {structurally stable}: given $f \in C^r(X_1 \times X_2,\mb{R})$, $g\in C^r(X_1 \times X_2,\mb{R})$, and a differential Nash equilibrium $(x_1,x_2) \in X_1 \times X_2$, there exists a neighborhoods $U \subset \mb{R}$ of zero and $V \subset X_1 \times X_2$ such that for all $t\in U$ there exists a unique differential Nash equilibrium $(\tilde x_1,\tilde x_2)  \in V$ for the zero-sum game $(f+tg,-f-tg)$. 
    \label{thm:ss_zsg}
\end{theorem}

\begin{proof}
	Define the smoothly perturbed cost function $\tilde f: X_1\times X_2 \times \mb{R} \rar \mb{R}$ by
	$\tilde f(x,y,t)=f(x,y)+tg(x,y)$,
 	and its differential game form $\tilde \omega:  X_1\times X_2 \times \mb{R} \rar T^*(X_1 \times X_2)$ by
 	\[ \tilde \omega(x,y,t)=(D_1(\tilde f(x,y)+tg(x,y),-D_2(\tilde f(x,y)+tg(x,y)),\]
 	for all $t \in \mb{R}$ and $(x,y) \in X_1 \times X_2$. 

 	Since $(x_1,x_2)$ is a differential Nash equilibrium, $D\tilde\omega(x,y,0)$ is necessarily non-degenerate (see the proof of Corollary~\ref{cor:hyperbolic}). Invoking the implicit function theorem~\cite{lee:2012aa}, there exists neighborhoods $V\subset \mb{R}$ of zero and $W \subset X_1 \times X_2$ and a smooth function $\sigma \in C^r(V,W)$ such that for all $ t \in V$ and $(x_1,x_2) \in W$, \[\tilde \omega(x_1,x_2,s)=0 \iff (x_1,x_2)=\sigma(t).\]

 	Since $\tilde \omega$ is continuously differentiable,
 	%$(x_1,x_2)=\sigma(t) \in V$,
 	%is necessarily a local Nash equilibrium. Further, 
 	there exists a neighborhood $U \subset W$ of zero such that $D\tilde \omega(\sigma(t),t)$ is invertible for all $t \in U$. Thus, for all $t \in U$, $\sigma(t)$ must be the unique Nash equilibrium of  $(f+tg|_W,-f-tg|_W)$. 
 	%Finally, since, for a fixed $t \in W$, $D\tilde \omega(\sigma(t),t)$ is invertible, $\sigma(t)$ must be an isolated differential Nash equilibrium. Thus, it must be the unique differential Nash equilibrium of $(f+tg|_V,-f-tg|_V)$.
\end{proof}
We note that both the genericity and structural stability results follow largely from the fact that the class of two-player zero-sum games are defined completely in terms of a single (sufficiently) smooth function $f\in C^r(X,\mb{R})$, so that its fairly straightforward to lift the properties of genericity and structural stability to the class of zero-sum games from the class of smooth functions. We also remark that the perturbations considered here are those such that the game remains in the class of zero-sum games; that is, the function $f$ is smoothly perturbed and this induces the perturbed zero sum game $(f+tg,-f-tg)$.

==> related_work.tex <==
\section{Related Work}
\label{sec:related_work}



==> theorems.tex <==
\section{Useful Theorems}

In order to prove genericity of non-degenerate differential Nash, we need some 
mathematical prelimiaries.

\subsection{Preliminaries}
Consider smooth manifolds $X$ and $Y$ of dimension $n_x$ and $n_y$ respectively.
An \emph{$k$--jet} from $X$ to $Y$ is an equivalence class $[x,\f,U]_k$ of
triples $(x,\f,U)$ where $U\subset X$ is an open set, $x\in U$, and $f:U\rar Y$
is a $C^k$ map. The equivalence relation satisfies $[x,\f,U]_k=[y,g,V]_k$ if
$x=y$ and in some (and hence any) pair of charts adapted to $\f$ at $x$, $\f$
and $g$ have the same derivatives up to order $k$. We use the notation
$[x,\f,U]_k=j^k\f(x)$ to denote the $k$--jet of $f$ at $x$. The set of all
$k$--jets from $X$ to $Y$ is denoted by $J^k(X,Y)$. The jet bundle $J^k(X, Y)$
is a smooth manifold (see \cite{Hirsch:1976la} Chapter 2 for the construction).
For each $C^k$ map $f:X\rar Y$ we define a map $j^kf:X\rar J^k(X, Y)$ by $x\mapsto j^kf(x)$ and refer to it as the \emph{$k$--jet extension}. 
%Suppose that $(U, \vphi)$ and $(V, \psi)$ are charts on $M$ and $N$ respectively. Let $\tilde{f}\in C^k(U, \mb{R}^n)$ Then $k$--jet of $\tilde{f}$ at $x\in U$
\begin{definition}
Let $X$, $Y$ be smooth manifolds and $f:X\rar Y$ be a smooth mapping. Let $Z$ be
a smooth submanifold of $Y$ and $p$ a point in $X$. Then \emph{$f$ intersects
$Z$ transversally at $p$} (denoted $f\pitchfork Z$ at $p$) if either $f(p)\notin
Z$ or $f(p)\in Z$ and $T_{f(p)} Y=T_{f(p)}Z + (f_\ast)_p(T_pX)$.
%\begin{enumerate}
%  \item $f(p)\notin Z$, or
%  \item $f(p)\in Z$ and $T_{f(p)} N=T_{f(p)}Z + (f_\ast)_p(T_pM)$.
%\end{enumerate}
\end{definition}

For $1\leq k<s\leq \infty$ consider the jet map 
%\begin{equation}
  $j^k:C^s(X, Y)\rar C^{s-k}(X, J^k(X, Y))$
%  \label{eq:jetmap}
%\end{equation}
and let $Z\subset J^k(X, Y)$ be a submanifold. 
Define
\begin{equation}
  \trans^s(X, Y; j^k, Z)=\{ h\in C^s(X, Y)|\ j^kh \pitchfork Z\}.
  \label{eq:jettrans}
\end{equation}
A subset of a topological space $X$ is \emph{residual} if it contains the intersection of countably many open--dense sets. We say a property is \emph{generic} if the set of all points of $X$ which possess this property is residual~\cite{broer:2010aa}. 
%\sam{Need def of strong topology.}

%We now introduce the \emph{strong topology} on $C^k(M, N)$. Let $\Phi=\{(U_i, \vphi_i)\}_{i\in I}$ be a locally finite set of charts on $M$ for some index set $I$. Let $K=\{K_i\}_{i\in I}$ be a family of compact subsets of $M$ such that $K_i\subset U_i$. Similarly, let $\Psi=\{(V_i, \psi_i)\}_{i\in I}$ be a family of charts on $N$ and $\{\vep_i\}_{i\in I}$ a family of positive numbers. Then, if $f\in C^k(M, N)$ takes each $K_i$ into $V_i$, then the set that contains all maps $g\in C^k(M, N)$ such that for all $i\in I$, $g(K_i)\subset V_i$ and 
%\begin{equation}
%  \|D^r(\psi_i\circ f\circ \vphi_i^{-1})(x)-D^r(\psi_i\circ g\circ \vphi_i^{-1})(x)\|\leq \vep_i
%  \label{eq:strongtop}
%\end{equation}
%for all $x\in \vphi_i(K_i)$, $r=0, \ldots, k$ is a \emph{strong basic neighborhood}. The strong topology has all possible sets of this form as its base.

%The following results will be used to prove genericity of non--degenerate differential Nash equilibria.

%{\it Theorem 2.8 in~\cite{Hirsch:1976la} \emph{(Jet Transversality)}}
\begin{theorem}(Jet Transversality Theorem, Chapter 2 of \cite{Hirsch:1976la}).
  Let $X$, $Y$ be $C^\infty$ manifolds without boundary, and let $Z\subset
  J^k(X, Y)$ be a $C^\infty$ submanifold. Suppose that $1\leq k<s\leq \infty$.
  Then, $\trans^s(X, Y; j^k, Z)$ is residual and thus dense in $C^s(X, Y)$ endowed with the strong topology, and open if $Z$ is closed. 
\label{thm:jettrans}
\end{theorem}
\begin{proposition}
  \label{prop:intersect}
  (Chapter II.4, Proposition 4.2~\cite{golubitsky:1973aa}). Let $X,Y$ be smooth
  manifolds and $Z\subset Y$ a submanifold. Suppose that $\dim X< \codim Z$. Let
  $f:X\rar Y$ be smooth and suppose that $f\pitchfork Z$. Then, $f(X)\cap Z=\emptyset$.
\end{proposition}
%In Section~\ref{sec:genericity}, we use an argument based on the co--dimension of the set of functions which do not have the properties we desire Theorem~\ref{thm:jettrans} allos
%The concepts introduced in this section are very important for the development of our main results. 

%The definition of residual set, and hence genericity, implies a notion of \emph{almost all} which will be necessary for showing that local Nash equilibria are generically non-degenerate differential Nash equilibria. 
%The latter have nice properties; they are isolated, structurally stable as we will see in Section~\ref{sec:stable}, and hence computable.

The Jet Transversality Theorem and Proposition~\ref{prop:intersect} can be used to show a subset of a jet bundle having a particular set of desired properties is generic. 
Indeed, consider the jet bundle $J^k(X, Y)$ and recall that it is a manifold
that contains jets $j^kf:X\rar J^k(X, Y)$ as its elements where $f\in C^k(X,
Y)$. Let $Z\subset J^k(X, Y)$ be the submanifold of the jet bundle that \emph{does not} possess the desired properties. 
If $\dim X<\codim\ Z$, then for a generic function $f\in C^k(X, Y)$ the image of the $k$--jet extension is disjoint from $Z$ implying that there is an open--dense set of functions having the desired properties. 
%We will use this argument in Section~\ref{sec:generic} to show that non--degenerate differential Nash equilibria are generic among local Nash equilibria. 


% \subsection{Hyperbolic Critical Points}
% \begin{theorem}
%     Critical points of vector fields are generically hyperbolic.     \label{thm:hyperbolic}
% \end{theorem}
% The above theorem is standard in dynamical systems theory. This implies that
% critical points of $\dot{x}=-\omega(x)$ for both general and zero-sum games are
% generically hyperbolic.
% \begin{proof}
%     Let $\mc{B}$ be the subset of matrices in which have at least one eigenvalue
%     on the imaginary axis. This is a semi-algebraic set. Indeed, 
%     \[\mc{B}^\ast=\{(A, t)|\ \det(A-itI)=0\}\]
%     is by definition an algebraic (hence semi-algebraic) subset of
%     $\mb{R}^{m\times m}\times\mb{R}$. Note that $\mc{B}$ is the projection of
%     $\mc{B}^\ast$ on to $\mb{R}^{m\times m}$. Since the image of a semi-algebraic set
%     under an algebraic map is at least semi-algebraic, then $\mc{B}$ is also
%     semi-algebraic. Since $\mc{B}$ has no interior points, it is the union of
%     submanifolds of co-dimension greater than or equal to one. 

%     Applying Theorem~\ref{thm:jettrans} for $1$-jet extensions to vector fields
%     as maps from $\mb{R}^m$ to itself. That is, we are considering a vector
%     field as a map taking $\mb{R}^m$ to $\mb{R}^m$ and considering its $1$-jet
%     extensions which are denoted by $J^1(\mb{R}^m, \mb{R}^m)$. Note that $J^1(\mb{R}^m, \mb{R}^m)$ can
%     be canonically identified with $\mb{R}^{m}\times \mb{R}^m\times
%     \mb{R}^{m\times m}$ so that the $1$-jet of $V$ at $x$ is identified with
%     $(x, V(x), DV(x))$. 

%     Consider $G_1=\mb{R}^m\times \{0\}\times\mc{B}$. From above, $G_1$ is the
%     union of submanifolds of codimensions greater than or equal to $m+1$. Hence,
%     $j^1V$ from $\mb{R}^m$ to $\mb{R}^m$ is transversal with respect to $G_1$ if
%     and only if the image of $j^1V$ is disjoint from $G_1$. The Jet
%     Transversality Theorem implies that for generic $C^r$ vector fields $V$ with
%     $r\geq 2$, the image of the $1$-jet extension $J^1(V)$ is disjoint from
%     $\mc{B}$ which gives the result that critical points being hyperbolic is a
%     generic property.
    
% \end{proof}




